Bursting bubbles in Herschel-Bulkley fluids: dynamics and jetting transitions

When a bubble rises to a free surface, its bursting dynamics in Newtonian fluids are governed by the interplay between viscous, capillary, and gravitational forces. In this work, we extend this classical problem to Herschel-Bulkley fluids, elucidating the role of viscoplasticity and non-Newtonian rheology in bubble bursting. Using direct numerical simulations validated against experiments, we systematically explore the influence of the key governing dimensionless parameters, such as the Bond number, the Ohnesorge number, the shear-dependent behavior and the plastocapillary number, each varied over several orders of magnitude. Our results reveal that viscoplasticity strongly controls the evolution and interaction of capillary waves within the cavity formed upon bubble rupture. Shear-thinning and shear-thickening effects are significant only for moderate Ohnesorge numbers, while at large Ohnesorge values the free surface dynamics converge to a non-flat equilibrium shape once the internal stresses fall below the yield stress. These findings provide new insights into the coupled effects of viscosity, gravity, yield stress, and shear-dependent rheology in multiphase flows, with broad implications for natural and industrial processes involving gas-liquid interfaces.

==> PreviousResults.tex <==
% This section presents a systematic analysis of the bursting dynamics of a bubble in a Herschel–Bulkley fluid. We vary the Bond number \( Bo \), the flow behavior index \( n \), and the plastocapillary number \( \mathcal{J} \) to explore their influence on capillary wave propagation, cavity collapse, jet formation, and droplet ejection. The dynamics are interpreted in the context of viscoplasticity, particularly how the yield stress and shear-thinning or thickening nature of the fluid modify classical bursting behavior.

We perform a comprehensive parametric study of bubble bursting in viscoplastic media, exploring the interplay between gravity, viscosity, shear-dependent rheology, and yield stress. The dynamics are governed by four key dimensionless groups: the Bond number ($Bo$), Ohnesorge number ($Oh$), power-law index ($n$), and a dimensionless yield-stress parameter ($\mathcal{J}$). We explore the range $0.001 < Oh < 1$, spanning from inertia-dominated to viscous-dominated regimes; $0.01 < Bo < 1$, where gravity significantly alters the initial bubble shape; $0.4 < n < 1.4$, covering both shear-thinning and shear-thickening behaviors; and $0 < \mathcal{J} < 0.8$, capturing the transition from Newtonian to strongly viscoplastic regimes. \CRCA{Note that we have run over 800 simulations to define this regime map.}

\CRCA{Before presenting the regime maps as a function of the different dimensionless groups,  figure~\ref{fig:x} illustrates three representative cases that we use to classify the 
interfacial phenomenology of the system for $n = 1.0$, $Oh_K = 0.01$, and $Bo = 0.01$.  The columns correspond to plastocapillary numbers $\mathcal{J} = 0.22$, $0.24$, and $0.26$, 
while the rows show successive times $t/\tau = 0.25$, $0.5$, $0.75$, and $1.0$.  The first case ($\mathcal{J}=0.22$) corresponds to the formation of a Worthington jet  followed by droplet ejection through an end-pinching mechanism. In the second case,  a vertical jet develops but no droplets detach; instead, the interface rises above the  bubble’s centre of mass. Finally, in the third case the interface never rises beyond the  centre of mass of the bubble.
}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.85\linewidth]{validation_frames/BH.eps}
%     \caption{Evolution of the cavity bottom height over time.}
%     \label{fig:cavity_bottom_height}
% \end{figure}


% Ohk=1, Ohk1e-0
% \OhkBoTimeFigure{Ohk1e-0}{Bo1e-0}{1}{1}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-0}{Bo1e-0}{1}{1}{07500}{0.75}
% \OhkBoTimeFigure{Ohk1e-0}{Bo1e-1}{1}{0.1}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-0}{Bo1e-1}{1}{0.1}{07500}{0.75}
% \OhkBoTimeFigure{Ohk1e-0}{Bo1e-2}{1}{0.01}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-0}{Bo1e-2}{1}{0.01}{07500}{0.75}

% Ohk=0.1, Ohk1e-1
% \OhkBoTimeFigure{Ohk1e-1}{Bo1e-0}{0.1}{1}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-1}{Bo1e-0}{0.1}{1}{07500}{0.75}
% \OhkBoTimeFigure{Ohk1e-1}{Bo1e-1}{0.1}{0.1}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-1}{Bo1e-1}{0.1}{0.1}{07500}{0.75}
% \OhkBoTimeFigure{Ohk1e-1}{Bo1e-2}{0.1}{0.01}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-1}{Bo1e-2}{0.1}{0.01}{07500}{0.75}

% Ohk=0.01, Ohk1e-2
% \OhkBoTimeFigure{Ohk1e-2}{Bo1e-0}{0.01}{1}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-2}{Bo1e-0}{0.01}{1}{07500}{0.75}
% \OhkBoTimeFigure{Ohk1e-2}{Bo1e-1}{0.01}{0.1}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-2}{Bo1e-1}{0.01}{0.1}{07500}{0.75}
% \OhkBoTimeFigure{Ohk1e-2}{Bo1e-2}{0.01}{0.01}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-2}{Bo1e-2}{0.01}{0.01}{07500}{0.75}

% Ohk=0.001, Ohk1e-3
% \OhkBoTimeFigure{Ohk1e-3}{Bo1e-0}{0.001}{1}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-3}{Bo1e-0}{0.001}{1}{07500}{0.75}
% \OhkBoTimeFigure{Ohk1e-3}{Bo1e-1}{0.001}{0.1}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-3}{Bo1e-1}{0.001}{0.1}{07500}{0.75}
% \OhkBoTimeFigure{Ohk1e-3}{Bo1e-2}{0.001}{0.01}{02500}{0.25}
% \OhkBoTimeFigure{Ohk1e-3}{Bo1e-2}{0.001}{0.01}{07500}{0.75}

\begin{figure}
    \centering
    \begin{tabular}{c c c}
        $\mathcal{J} = 0.22$ & $\mathcal{J} = 0.24$ & $\mathcal{J} = 0.26$ \\
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/1_02500.png} &
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/2_02500.png} &
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/3_02500.png} \\
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/1_05000.png} &
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/2_05000.png} &
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/3_05000.png} \\
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/1_07500.png} &
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/2_07500.png} &
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/3_07500.png} \\
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/1_10000.png} &
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/2_10000.png} &
        \includegraphics[width=0.32\textwidth]{BubbleDynamics/Frames/3_10000.png} \\
    \end{tabular}
    \caption{
    Burst dynamics for $n = 1.0$, $Oh_K = 0.01$, and $Bo = 0.01$.
    Columns show plastocapillary number $\mathcal{J} = 0.22$, $0.24$, $0.26$;
    rows correspond to times $t/\tau = 0.25$, $0.5$, $0.75$, and $1.0$. \CRCAr{It is not clear the formation of droplets}
}
\label{fig:bursting_dynamics}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{RegimeMaps/OhK1e-0.eps}
%     \caption{Regime map of bubble bursting dynamics in the $(\log_{10} Bo, \mathcal{J}, n)$ space at $Oh_K = 1$. 
%     Color coding: 
%     \textcolor[rgb]{0.545, 0.271, 0.075}{brown} = no jet no drop; 
%     \textcolor[rgb]{1.000, 0.647, 0.000}{orange} = jet no drop; 
%     \textcolor[rgb]{0.118, 0.565, 1.000}{blue} = jet and drop.}
%     \label{fig:regime_ohk1}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{RegimeMaps/OhK1e-1.eps}
%     \caption{Regime map of bubble bursting dynamics in the $(\log_{10} Bo, \mathcal{J}, n)$ space at $Oh_K = 0.1$. 
%     Color coding: 
%     \textcolor[rgb]{0.545, 0.271, 0.075}{brown} = no jet no drop; 
%     \textcolor[rgb]{1.000, 0.647, 0.000}{orange} = jet no drop; 
%     \textcolor[rgb]{0.118, 0.565, 1.000}{blue} = jet and drop.}
%     \label{fig:regime_ohk01}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{RegimeMaps/OhK1e-2.eps}
%     \caption{Regime map of bubble bursting dynamics in the $(\log_{10} Bo, \mathcal{J}, n)$ space at $Oh_K = 0.01$. 
%     Color coding: 
%     \textcolor[rgb]{0.545, 0.271, 0.075}{brown} = no jet no drop; 
%     \textcolor[rgb]{1.000, 0.647, 0.000}{orange} = jet no drop; 
%     \textcolor[rgb]{0.118, 0.565, 1.000}{blue} = jet and drop.}
%     \label{fig:regime_ohk001}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\textwidth]{RegimeMaps/OhK1e-3.eps}
%     \caption{Regime map of bubble bursting dynamics in the $(\log_{10} Bo, \mathcal{J}, n)$ space at $Oh_K = 0.001$. 
%     Color coding: 
%     \textcolor[rgb]{0.545, 0.271, 0.075}{brown} = no jet no drop; 
%     \textcolor[rgb]{1.000, 0.647, 0.000}{orange} = jet no drop; 
%     \textcolor[rgb]{0.118, 0.565, 1.000}{blue} = jet and drop.}
%     \label{fig:regime_ohk0001}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\textwidth]{RegimeMaps/map.eps} % Update path/filename as needed
    \caption{Regime map of bubble bursting dynamics in the $(\mathcal{J}, n)$ space for various Bond numbers $Bo$ at fixed Ohnesorge number $Oh_K = 0.01$. Each subplot corresponds to a unique $(Oh_K, Bo)$ combination. 
    Color coding: 
    \textcolor[rgb]{0.545, 0.271, 0.075}{brown} = no jet, no drop; 
    \textcolor[rgb]{1.000, 0.647, 0.000}{orange} = jet, no drop; 
    \textcolor[rgb]{0.118, 0.565, 1.000}{blue} = jet and drop.}
    \label{fig:regime_ohk001}
\end{figure}

Figure~\ref{fig:regime_ohk001} summarizes the bursting outcomes in the 
$(\mathcal{J},n)$ space for different $(Oh_K,Bo)$ combinations. 
\CRCA{The regime map shows the close interplay between capillarity, gravitational forces, viscous dissipation and yield stress.}

\CRCA{In the upper-left corner of parameter space, corresponding to low $J$, low-to-moderate $Oh_K$, and small $Bo$, capillarity dominates to generate slender jets that often culminate in droplet detachment. Moving horizontally toward larger $J$, viscoplastic stresses increasingly oppose deformation, suppressing the collapse and leading to trivial relaxations without jetting. Vertically upward in $n$, as fluids move from shear-thinning to Newtonian and finally shear-thickening behavior, the enhanced viscous resistance further damps the cavity collapse of the bubble, transforming jetting-with-drop regimes into jets without drops, and eventually to no jet at all. Increasing the Ohnesorge number shifts the balance toward viscous dominance; at moderate $Oh_K$, only shear-thinning fluids retain enough mobility to sustain jetting, while at $Oh_K=1$ viscous stresses overwhelm all capillary-driven cavity collapse, and no jets are observed anywhere in the map. }

\CRCA{The overall structure of the map thus conveys a simple physical picture: bubble bursting dynamics are confined to a narrow region of parameter space where capillarity is able to overcome both viscous and gravitational resistance. Inertia and shear-thinning promote jet focusing and droplet detachment, while gravity and high viscosity act to choke the recoil, yielding a smooth relaxation of the free surface. }

\CRCA{
We note that the previous work by Vatsal presented a regime map in the $(J,Oh)$ space for a very weak-gravity case ($Bo=10^{-3}$). In our maps we step up gravity by one to three decades ($Bo=10^{-2},10^{-1},10^{0}$), and the trend changes significantly compared to the previous work by Vatsal. As $Bo$ increases, the shape of the bubble deviates from spherical, leading to a pre-flattened cavity that opposes the capillary collapse responsible for the formation of the Worthington jet. No formation of droplets is predicted below $\mathrm{La}=500$ (or equivalently for $Oh>0.044$), independent of the Bond number in the range $10^{-3}\leq Bo \leq 10$, which agrees with our observations (see Berni et al.). }

\CRCA{
Taken together, increasing $Bo$ acts like adding ``effective damping'' on top of $Oh$ and $J$: it lowers jet speeds, shortens jet heights, and suppresses cavity collapse. In our regime maps this is exactly what we see across the columns: the jet + drop regime collapses to yellow (jet only), then to brown (no jet) as $Bo$ grows, with all boundaries shifting left/down in $(J,Oh)$ space and toward more shear-thinning as $n$ varies.}




At the largest Ohnesorge number ($Oh_K=1$), all cases remain in the 
brown regime, corresponding to fully arrested dynamics with no jet 
formation. In this strongly viscous limit, inertial focusing is completely 
suppressed regardless of $\mathcal{J}$ or $n$. 

As $Oh_K$ is reduced, inertial effects become more prominent and transitions 
to jetting (orange and blue states) begin to appear. A similar trend is observed 
when lowering the Bond number, which reduces gravitational suppression and 
enhances capillary focusing. These transitions first occur at intermediate 
values of $(Oh_K,Bo)$, where a competition between viscoplastic stresses and 
capillary--inertial dynamics produces mixed outcomes. To better resolve the 
phenomenology in these transitional regions, additional simulations were 
performed around the critical values of $\mathcal{J}$ and $n$. 

Within a fixed $(Oh_K,Bo)$ pair, the regime boundaries follow systematic trends. 
Decreasing $\mathcal{J}$ lowers the yield-stress barrier, enabling wave 
propagation, cavity collapse, and ultimately jet formation. Similarly, reducing 
$n$ (shear-thinning behavior) decreases the effective viscosity in regions of 
large strain rate, thereby favoring jet emergence. As a result, the progression 
from brown $\rightarrow$ orange $\rightarrow$ blue corresponds physically to 
a gradual release of viscoplastic constraints: first allowing a jet to form, and 
then allowing sufficient focusing for droplet pinch-off. 

% --- First Row: Varying n (Folders 1–3) ---
\begin{figure}
    \centering
    \includegraphics[width=0.32\textwidth]{CavityDynamics/1.eps} \hfill
    \includegraphics[width=0.32\textwidth]{CavityDynamics/2.eps} \hfill
    \includegraphics[width=0.32\textwidth]{CavityDynamics/3.eps}
    \caption{Effect of varying $n$ on cavity dynamics for fixed $\mathcal{J}$, $Bo$, and $Oh_K$.}
    \label{fig:varying_n}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.72\linewidth]{Shapes.eps}
    \caption{Cavity shapes at $t/\tau = 0.5$ for $Oh_K = 0.1$, $\mathcal{J} = 0.06$, and $Bo = 0.01$.
    Curves correspond to $n \in \{0.4, 0.6, 0.8, 1.0, 1.2, 1.4\}$.}
    \label{fig:shapes}
\end{figure}

Across all three panels of figure~\ref{fig:varying_n}, the early-time response and the long-time relaxation of the cavity height are essentially insensitive to the flow index $n$. The differences induced by $n$ appear in the intermediate window when the capillary wave reaches the axis and the cavity shoots upward. As $n$ decreases (stronger shear--thinning), two systematic trends emerge: 
(i) the transition to the rapid-rise segment becomes sharper and less damped, with a larger slope $\,\mathrm{d}Z_b/\mathrm{d}t\,$ and a more pronounced overshoot; 
(ii) the maximum cavity height $Z_{b,\max}$ increases monotonically. 
Physically, the effective viscosity in a Herschel--Bulkley fluid scales as $\mu_{\mathrm{eff}}\sim(2\|\mathcal{D}\|+\varepsilon)^{\,n-1}$; thus, for $n<1$ the regions of large strain rate near the cavity neck experience a strong viscosity reduction, which lowers dissipation, enlarges the yielded zone, and enhances capillary–inertial focusing. For $n>1$ (shear--thickening), the opposite occurs: dissipation increases and the focusing is damped, smoothing the transition and limiting $Z_{b,\max}$.

Figure~\ref{fig:shapes} compares instantaneous cavity profiles for fixed $Oh_K=0.1$, $\mathcal{J}=0.06$, and $Bo=0.01$. Decreasing $n$ straightens the cavity sidewalls, producing a more columnar shape, whereas increasing $n$ yields smoother, more curved flanks. This morphology reflects how shear--thinning localizes deformation: at low $n$ the high-strain region remains confined near the axis, leaving the outer flanks weakly sheared (and partly unyielded), which favors nearly linear sidewalls; at higher $n$ the dissipation is larger and the yielded region spreads, distributing curvature more uniformly along the interface.


% --- Second Row: Varying J (Folders 4–5) ---
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{CavityDynamics/4.eps} \hfill
    \includegraphics[width=0.48\textwidth]{CavityDynamics/5.eps}
    \caption{Effect of varying $\mathcal{J}$ on cavity dynamics for fixed $n$, $Bo$, and $Oh_K$.}
    \label{fig:varying_J}
\end{figure}

Figure~\ref{fig:varying_J} illustrates the influence of the plastocapillary number $\mathcal{J}$ 
on the evolution of cavity height for fixed $n$, $Bo$, and $Oh_K$. In both cases, decreasing 
$\mathcal{J}$ allows the cavity to rise to a larger overshoot, reaching a well-defined maximum 
before relaxing back toward equilibrium. As $\mathcal{J}$ increases, this overshoot is progressively 
suppressed: the maximum cavity height diminishes, the peak occurs later in time, and the subsequent 
relaxation is less pronounced. Beyond a critical $\mathcal{J}$, the overshoot vanishes entirely, 
and the cavity rises monotonically to a lower asymptotic height without producing a distinct maximum. 

This behavior reflects the competing roles of capillary focusing and yield stress. At small 
$\mathcal{J}$, capillary stresses dominate, driving a rapid cavity collapse that launches the 
interface upward. At large $\mathcal{J}$, the yield stress resists deformation and prevents 
the cavity from fully focusing, thereby damping vertical motion and reducing the attainable 
cavity height. Consequently, increasing $\mathcal{J}$ not only lowers the peak amplitude of 
the cavity but also reduces its final steady-state position.

% \begin{enumerate}
%     \item $Oh_k=0.1$, J=[0.02,0.04, 0.06, 0.08]
%     
%     \item $Oh_k=0.01$
%     \begin{enumerate}
%         \item Bo=1, J=[0.12,0.14, 0.16, 0.18]
%         \item Bo=[0.1, 0.01], J=[0.22,0.24, 0.26, 0.28]
%         \item Bo=0.5, J=[0,0.1,0.2,0.3]
%     \end{enumerate}
%     \item $Oh_k=0.001$:
%     \begin{enumerate}
%         \item Bo=1, J=[0.12,0.14, 0.16, 0.18]
%         \item Bo=[0.1, 0.01, 0.001], J=[0.22,0.24, 0.26, 0.28]
%         \item Bo=0.5, J=[0,0.1,0.2,0.3]        
%     \end{enumerate}
% \end{enumerate}

The bursting of a bubble in a viscoplastic medium proceeds through a sequence of interrelated events following the removal of the cap. Initially, capillary waves are generated at the cavity edge and propagate along the free surface. These waves converge at the axis of symmetry, leading to cavity collapse and the formation of a central jet. The nature of these stages—wave propagation, cavity dynamics, and jetting—is strongly influenced by the fluid’s viscoplastic properties. Depending on the plastocapillary number $\mathcal{J}$, Bond number $Bo$, and flow behavior index $n$, the outcome can range from classical inertial jetting to fully arrested dynamics with no ejection. The following sections detail the role of each parameter in shaping these behaviors.

Capillary waves are initiated immediately after the rupture of the thin film separating the bubble from the free surface. In Newtonian fluids, such waves travel freely and symmetrically, ultimately converging to form a Worthington jet. In viscoplastic fluids, however, yield stress and non-Newtonian viscosity dampen the wave propagation. We analyze the spatiotemporal evolution of the interface and extract the maximum curvature location to track the strongest wave. The effect of increasing $\mathcal{J}$ and varying $n$ on wave attenuation and phase speed is highlighted. 

\begin{figure}
    \centering
    \begin{tabular}{@{}c c@{}}
        \includegraphics[width=0.48\textwidth]{CapillaryWaves/1.eps} &
        \includegraphics[width=0.48\textwidth]{CapillaryWaves/2.eps} \\
        \includegraphics[width=0.48\textwidth]{CapillaryWaves/3.eps} &
        \includegraphics[width=0.48\textwidth]{CapillaryWaves/4.eps} \\
    \end{tabular}
    \caption{Effects of viscoplasticity on the travelling capillary waves.}
    \label{fig:capillary_waves}
\end{figure}

Figure~\ref{fig:capillary_waves} quantifies these dynamics by tracking four capillary--wave point characteristics: 
(a) the curvature magnitude $|\kappa_c|$, 
(b) the radial position $R_c$ relative to the symmetry axis, 
(c) the vertical location $Z_c$, and 
(d) the arclength $s_c$ measured from the cavity bottom to the wave crest. 
Across all cases, $|\kappa_c|$ initially decreases as the highly curved rim relaxes after rupture. 
At low $\mathcal{J}$, the wave subsequently focuses toward the axis, producing renewed curvature growth, 
whereas at high $\mathcal{J}$, viscoplastic resistance suppresses this focusing and curvature remains nearly constant. 
A similar trend is observed in the radial position $R_c$: after an initial outward motion, the crest turns inward, 
with stronger migration at small $\mathcal{J}$ and a near-arrested motion at large $\mathcal{J}$. 
The vertical position $Z_c$ decreases monotonically, indicating that the crest penetrates deeper into the cavity, 
again more strongly at low $\mathcal{J}$. 
Finally, the arclength $s_c$ decreases as the capillary wave moves closer to the cavity apex; 
this contraction is pronounced at small $\mathcal{J}$ and weak at large $\mathcal{J}$. 
Taken together, these metrics show that decreasing $\mathcal{J}$ promotes capillary–inertial focusing, 
while increasing $\mathcal{J}$ damps wave propagation and can prevent the focusing that precedes jet formation.

